Machine-Learning Side-Channel Attacks on the GALACTICS Constant-Time Implementation of BLISS

Due to the advancing development of quantum computers, practical attacks on conventional public-key cryptography may become feasible in the next few decades. To address this risk, post-quantum schemes that are secure against quantum attacks are being developed. Lattice-based algorithms are promising replacements for conventional schemes, with BLISS being one of the earliest post-quantum signature schemes in this family. However, required subroutines such as Gaussian sampling have been demonstrated to be a risk for the security of BLISS, since implementing Gaussian sampling both efficient and secure with respect to physical attacks is highly challenging. This paper presents three related power side-channel attacks on GALACTICS, the latest constant-time implementation of BLISS. All attacks are based on leakages we identified in the Gaussian sampling and signing algorithm of GALACTICS. To run the attack, a profiling phase on a device identical to the device under attack is required to train machine learning classifiers. In the attack phase, the leakages of GALACTICS enable the trained classifiers to predict sensitive internal information with high accuracy, paving the road for three different key recovery attacks. We demonstrate the leakages by running GALACTICS on a Cortex-M4 and provide proof-of-concept data and implementation for all our attacks.

==> Rebuttal.tex <==
Rebuttal Phase
============================================
Answer to the First Review
============================================
We embedded the information obtained by the side-channels in a linear system and did not consider the lattice structure of the secret key into account. We believe that the easiest way is to require exact knowledge and build a system of linear equations to determine the secret key. This method comes at the expense of more signatures but has a high-speed and efficient offline part (milliseconds) compared to lattice reduction algorithms such as LLL.

The probability that x>3 is 0,02. The frequency of these values in the training data is low. It is challenging to train the model for the correct prediction of these values.  
To add an equation holding a false x (with x>3) to our linear system, we should satisfy the two conditions: yu = 0 and x>3. The probability that yu=0 is 0,4. Hence, the probability of having a false equation is 0,4 multiplied by 0,02, which is very low and does not affect the correctness of the retrieved secret key. 

============================================
Answer to the Second Review
============================================
We signed a number of uniform randomly chosen messages using random, individual keys to prepare the profiling. To prepare the attack, the key pair generation was invoked to generate the key under attack and a number of uniform randomly chosen, attacker-known messages were signed.  
============================================
Answer to the Third Review
============================================
BLISS is an old scheme, but it has seen a first real-world adoption in strongSwan, an IPsec-based VPN. Moreover, the BLISS scheme has a better performance than all the NIST candidates. It was eliminated from the NIST because of its security vulnerability due to the use of the Gaussian sampling. The implementation-security aspects of BLISS have been the focus of many research work in literature. 

The first two attacks we presented against BLISS target one of the latest implementations of the CDT and the Bernoulli sampler [2]. Those subroutines (and the implementation in [2]) are excessively used in lattice-based schemes in general and specifically NIST candidates (e.g., FrodoKEM, FALCON). Our attacks can be applied to NIST candidates using the targeted subroutines; the secret key retrieval algorithms defined in section 6 must be adapted to the attacked algorithm. However, this is not the scope of our paper.

For our experiments, we opted for a commonly used setup consisting of the ChipWhisperer-Lite board, the CW308 UFO board, and the CW308T-STM32F4 target board. This setup has been used in most previous research papers to present a proof of concept implementation of a side-channel attack. An example that can be cited is the recent paper [3], where the target board runs 24 MHz.  
============================================
Answer to the Fourth Review
============================================
\item \textbf{Fourth review: } 
Our choice for hyperparameter was selected using the grid search algorithm, which trains a model for every possible combination of hyperparameter values in the set of values for each individual hyperparameter [1].

We tested whether our solution can be simplified in different ways. We defined "Trivial prediction accuracy" which is achieved by always predicting the most likely label, "linear accuracy" by using a single-layer perceptron, and "MLP accuracy" by using a multi-layer perceptron. We showed in Table 2 that the use of the MLP method provides the best prediction accuracy for all the leakages we defined. 
 
[1]  Ian Goodfellow, Yoshua Bengio, and Aaron Courville. 2016. Deep Learning. MIT671
Press. http://www.deeplearningbook.org.6
[2] https://eprint.iacr.org/2018/1234.pdf
[3] https://tches.iacr.org/index.php/TCHES/article/view/9079

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.46586/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}


==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.46586/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

